$\lambda$FS: A Scalable and Elastic Distributed File System Metadata Service using Serverless Functions

The metadata service (MDS) sits on the critical path for distributed file system (DFS) operations, and therefore it is key to the overall performance of a large-scale DFS. Common "serverful" MDS architectures, such as a single server or cluster of servers, have a significant shortcoming: either they are not scalable, or they make it difficult to achieve an optimal balance of performance, resource utilization, and cost. A modern MDS requires a novel architecture that addresses this shortcoming. To this end, we design and implement $\lambda$FS, an elastic, high-performance metadata service for large-scale DFSes. $\lambda$FS scales a DFS metadata cache elastically on a FaaS (Function-as-a-Service) platform and synthesizes a series of techniques to overcome the obstacles that are encountered when building large, stateful, and performance-sensitive applications on FaaS platforms. $\lambda$FS takes full advantage of the unique benefits offered by FaaS $\unicode{x2013}$ elastic scaling and massive parallelism $\unicode{x2013}$ to realize a highly-optimized metadata service capable of sustaining up to 4.13$\times$ higher throughput, 90.40% lower latency, 85.99% lower cost, 3.33$\times$ better performance-per-cost, and better resource utilization and efficiency than a state-of-the-art DFS for an industrial workload.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> __related_work_101522.tex <==
\vspace{-4pt}
\section{Related Work}
\label{sec:related}
\vspace{-2pt}

% yue: Backed up with richer text just in case later we need the text for other purposes.

%\noindent\textbf{High-performance MDS.}
InfiniFS~\cite{InfiniFSEfficientMetadata} is a metadata service for large-scale DFS. InfiniFS decouples access and content directory metadata in order to implement a partitioning scheme that considers both locality and load balancing. They also implement a technique referred to as \textit{speculative path resolution} to optimize path resolutions by performing them in-parallel. This can lead to reduced per-operation latency. Finally, they use a client-side ``optimistic access metadata cache'' to mitigate the near-root hotspot issue. This technique leads to improved system throughput. \textcolor{red}{{\proj} does not utilize speculative path resolution, instead opting to use HopsFS' existing \textit{INode Hint Cache} to optimize path resolution. {\proj} also elects to use server-side caching atop serverless functions rather than client-side caching.}

IndexFS~\cite{indexfs_sc14} is a distributed file system designed and optimized for metadata workloads with many small files. IndexFS is considered a middleware file system, as it is built atop existing DFS (e.g., HDFS~\cite{hdfs_msst10}). Metadata servers are responsible for serving metadata requests and user data requests for small files stored using LevelDB~\cite{leveldb}. Larger files are managed by the underlying DFS. 
%IndexFS does not support atomic operations involving both itself and the underlying DFS. 
IndexFS supports metadata caching in order to optimize the performance of frequently-accessed files and directories. \yuec{Compared with IndexFS, {\proj} enables horizontal MDS elasticity using serverless functions and uses a lightweight consistency protocol to guarantee consistency across serverless functions.} 
%\yuec{add GIGA+. diff?}

LocoFS~\cite{locoFS} co-locates all metadata from a single directory on the same metadata server\textcolor{red}{, similar to how {\proj}'s partitioning mechanism will colocate metadata from single directories within single deployments.} This reduces the latency for path resolutions, which can boost performance. This caching system can lead to single-node bottlenecks, however, as a single metadata server can end up serving all metadata requests for a hot directory. \textcolor{red}{{\proj} avoids this bottleneck by taking advantage of the horizontal elasticity of serverless computing to scale-out the deployments responsible for caching metadata of hot directories.}

Other DFSes instead use pure hashing that hashes on 
%hash on file or directory names 
file name or full pathname. Examples include Lustre~\cite{lustre}, CalvinFS~\cite{thomsonCalvinFSConsistentWAN2015}, BetrFS~\cite{jiaoBetrFSCompleatFile2022}, and Giraffa~\cite{ScalingNamespaceOperations}. Lustre hashes on the file name.
CalvinFS hashes on the full pathname, while Giraffa uses full file paths as primary keys to the associated metadata. BetreFS uses the pathname as a file index into the local file system. These strategies can result in increased implementation complexity and reduced performance~\cite{InfiniFSEfficientMetadata}. 
Lazy Hybrid~\cite{lh_msst03} combines both directory subtree management and hashing-based approach with lazy metadata relocation and lazily updated dual-entry access control lists (ACLs). \yuec{diff?}

%Finally, ZooKeeper~\cite{ApacheZooKeeper} is a centralized synchronization service. ZooKeeper can be used for naming, distributed synchronization, group services, and managing configuration information. 

%\noindent\textbf{Serverless Caches and Storage.}
\textsc{InfiniCache}~\cite{infinicache_fast20} exploits the collective memory of AWS Lambda functions to cache data objects. 
OFC~\cite{ofc_eurosys21} is an opportunistic memory cache that leverages overbooked host memory of serverless functions to accelerate function execution. 
Faa\$T~\cite{faast_socc21} is a distributed cache that is co-located with a FaaS application. Faa\$T scales as the FaaS application scales.
%Pocket~\cite{pocket_osdi18, ephemeral_atc18} is an elastic ephemeral storage for serverless analytics~\cite{pywren_socc17, locus_nsdi19}. SONIC~\cite{sonic_atc21} optimizes data exchanging among chained functions.
AFT~\cite{aft_eurosys20} is a fault-tolerant shim that provides atomic transaction guarantees to serverless applications that store data in cloud storage. 
% Faa\$T~\cite{faast_socc21} is an auto-scaled, distributed cache that is co-located with serverless function applications. 
% In contrast, {\proj} leverages serverless functions to achieve rapid scaling while providing highly available data accesses.
Shedder~\cite{shredder_socc19} moves function computation directly to cloud storage.
Pocket~\cite{pocket_osdi18} and Jiffy~\cite{jiffy_eurosys22} provide elastic, serverful, ephemeral storage for serverless analytics.
{\proj} uses the memory resource of serverless functions but as a consistent, distributed metadata cache for DFS workloads. 

==> eqn_annotate.tex <==
\usepackage{tikz}
\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{mathtools, nccmath}
\usepackage{wrapfig}
\usepackage{comment}

% To generate dummy text
\usepackage{blindtext}


%color
%\usepackage[dvipsnames]{xcolor}
% \usepackage{xcolor}


%\usepackage[pdftex]{graphicx}
\usepackage{graphicx}
% declare the path(s) for graphic files
%\graphicspath{{../Figures/}}

% extensions so you won't have to specify these with
% every instance of \includegraphics
% \DeclareGraphicsExtensions{.pdf,.jpeg,.png}

% for custom commands
\usepackage{xspace}

% table alignment
\usepackage{array}
\usepackage{ragged2e}
\newcolumntype{P}[1]{>{\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{X}[1]{>{\RaggedRight\hspace*{0pt}}p{#1}}

% color box
\usepackage{tcolorbox}


% for tikz
\usepackage{tikz}
%\usetikzlibrary{trees}
\usetikzlibrary{arrows,shapes,positioning,shadows,trees,mindmap}
% \usepackage{forest}
\usepackage[edges]{forest}
\usetikzlibrary{arrows.meta}
\colorlet{linecol}{black!75}
\usepackage{xkcdcolors} % xkcd colors


% for colorful equation
\usepackage{tikz}
\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}
% Commands for Highlighting text -- non tikz method
\newcommand{\highlight}[2]{\colorbox{#1!17}{$\displaystyle #2$}}
%\newcommand{\highlight}[2]{\colorbox{#1!17}{$#2$}}
\newcommand{\highlightdark}[2]{\colorbox{#1!47}{$\displaystyle #2$}}

% my custom colors for shading
\colorlet{mhpurple}{Plum!80}


% Commands for Highlighting text -- non tikz method
\renewcommand{\highlight}[2]{\colorbox{#1!17}{#2}}
\renewcommand{\highlightdark}[2]{\colorbox{#1!47}{#2}}

% Some math definitions
\newcommand{\lap}{\mathrm{Lap}}
\newcommand{\pr}{\mathrm{Pr}}

\newcommand{\Tset}{\mathcal{T}}
\newcommand{\Dset}{\mathcal{D}}
\newcommand{\Rbound}{\widetilde{\mathcal{R}}}

==> eval_old.tex <==
\vspace{-4pt}
\section{Evaluation}
\label{sec:eval}
\vspace{-8pt}

%\subsection{{\proj}}
%\label{sec:eval_serverless_mds}

\subsection{Experimental Setup \& Methodology}
\label{subsec:eval_methodology}
\vspace{-6pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Weak Scaling Throughput Figure %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[t]
% %\vspace{-5pt}
% \begin{center}

% \subfigure[Read file.] {
% \includegraphics[width=0.18\textwidth]{graphs/weak_scaling/weak_read.pdf}
% \label{fig:l_ws_read}
% }
% \hspace{-8pt}
% \subfigure[Stat file.] {
% \includegraphics[width=0.18\textwidth]{graphs/weak_scaling/weak_stat.pdf}
% \label{fig:l_ws_stat}
% }
% \hspace{-8pt}
% \subfigure[List directory.] {
% \includegraphics[width=0.18\textwidth]{graphs/weak_scaling/weak_ls.pdf}
% \label{fig:l_ws_ls_dir}
% }
% \hspace{-8pt}
% \subfigure[Create file.] {
% \includegraphics[width=0.18\textwidth]{graphs/weak_scaling/weak_create_file.pdf}
% \label{fig:l_ws_create_file}
% }
% \hspace{-8pt}
% \subfigure[Create directory.] {
% \includegraphics[width=0.18\textwidth]{graphs/weak_scaling/weak_mkdir.pdf}
% \label{fig:l_ws_mkdir}
% }
% \vspace{-10pt}
% \caption{\textit{Client-driven} scaling comparison between {\proj} and HopsFS. The total amount of vCPUs allocated to {\proj} and HopsFS was held constant at 512 vCPUs, and each client performed 2,048 operations. The number of clients ranged from 8 to 1,024.}
% \label{fig:weak_scale_throughput}
% \vspace{-16pt}
% \end{center}
% \end{figure*}

\addcomment{In order to elucidate the effectiveness of {\proj}'s various techniques and optimizations, we evaluated {\proj} against a number of other file systems. Specifically, we compared {\proj} against three state-of-the-art distributed file systems: HopsFS, IndexFS~\cite{indexfs_sc14}, and CephFS~\cite{ceph_mds_sc04}. We also performed experiments that evaluated {\proj} against that of a modified HopsFS, denoted ``HopsFS+Cache'', whose NameNodes had been augmented with an in-memory metadata cache similar to that of {\proj}. HopsFS+Cache serves as a serverful, cache-based DFS baseline. Finally, we compared {\proj} with {\infcache}~\cite{infinicache_fast20}, an in-memory object cache implemented atop FaaS, in order to better understand the efficacy of {\proj}'s FaaS caching layer. All experiments were performed on Amazon Web Services (AWS). The results of the experiments were also verified to be consistent with results obtained on Google Cloud Platform (GCP).}

%\addcomment{All experiments were performed on Google Cloud Platform (GCP) and Amazon Web Services (AWS). OpenWhisk was deployed on Google Kubernetes Engine (GKE) and AWS Elastic Kubernetes Service (EKS). All other VMs were deployed on Google Compute Engine (GCE) and AWS EC2. All AWS VMs used the \texttt{\small{r5.4xlarge}} instance type (16 vCPU and 128GB RAM), while all GCP VMs (GCE and GKE) used the \texttt{\small{r5.4xlarge}} instance type (16 vCPU and 64GB RAM). These instance types were selected because they exhibit similar performance and have similar hardware configurations. For example, both instance families use second generation Intel Xeon Scalable processors (Cascade Lake)~\cite{google-c2-instance-family, amazon-r5-instance-family}.}

\addcomment{The experiments used deployments of the OpenWhisk serverless platform and MySQL Cluster NDB. Like {\proj}, HopsFS uses MySQL Cluster NDB as its persistent metadata store. OpenWhisk was deployed on AWS Elastic Kubernetes Service (EKS). All other VMs were deployed on AWS EC2. All AWS VMs used the \texttt{\small{r5.4xlarge}} instance type (16 vCPU and 128GB RAM). MySQL Cluster NDB 8.0.26 was deployed on GCE and EC2 with a single master node and four data nodes. We configured each NDB storage node according to the sample configuration provided by HopsFS. Unless otherwise specified, %each {\proj} NameNode is configured with 5 vCPU and 19GB RAM, and 
each {\proj} NameNode was configured with 6.25 vCPU and 30GB RAM. HopsFS' NameNodes were configured with 16 vCPU, 64GB RAM, and 200 RPC handlers.} For clarity, we defer the description of the \diffcomment{setup for the portability experiment}{portability experiment setup} with IndexFS to \cref{sec:indexfs-results} as IndexFS' architecture is different from HopsFS.
 
%\delcomment{All experiments were performed on Google Cloud Platform (GCP). OpenWhisk was deployed on Google Kubernetes Engine (GKE). %OpenWhisk was configured to use 2 \texttt{\small{Controller}} replicas and 3 \texttt{\small{Invoker}} replicas. 
%Client VMs and DataNodes (for both {\proj} and HopsFS) were deployed on Google Compute Engine (GCE), as were HopsFS' NameNodes. We also deployed MySQL Cluster NDB 8.0.26 on GCE with a single manager node and four data nodes. Like {\proj}, HopsFS uses MySQL Cluster NDB as its persistent metadata store. We configured each NDB storage node according to the sample configuration provided by HopsFS. All VMs used the \texttt{\small{c2-standard-16}} instance type, which has 16 vCPUs and 64GB RAM.}
%\added{
%\delcomment{Each of {\proj}' individual serverless NameNodes was configured with 5 vCPUs and 19GB of RAM unless otherwise specified. Each of HopsFS' NameNodes was configured to use 200 RPC handler threads.}
%} 
 %\delcomment{Finally, {\proj}'s \textit{ConcurrencyLevel} and \textit{TcpHttpReplacement\%} parameters were set to \diffcomment{2}{3} and \diffcomment{0.0035}{0.003}, respectively.}
%For additional information about all of the framework configurations, please refer to our open-source benchmarking repository~\cite{lambda-mds-benchmark-app-anonymous}.

%In order 
To ensure a fair comparison between {\proj} and HopsFS, we allocated an equal amount of vCPUs and RAM to each framework's NameNode cluster (unless otherwise specified). \diffcomment{However, it is important to point out that}{However,} statically provisioning a fixed amount of vCPUs for {\proj}' NameNodes implicitly limited the maximum performance \diffcomment{compared to the performance {\proj} could have achieved with}{that {\proj} could achieve compared to {\proj}' performance with} the nearly unbounded resources typically provided by FaaS platforms. %Because of the bound on vCPUs, 
Because of this bound \addcomment{on vCPUs},
unrestricted {\proj} scale-outs would have over-used resources, leading to thrashing and severe performance degradation. To \diffcomment{prevent}{address} this, {\proj}' scaling behavior was ``toned down'', and consequently {\proj} never used more than \diffcomment{87.8\%}{79\%} of the available vCPUs during these experiments. (We \diffcomment{describe}{introduce} {\proj}' anti-thrashing technique in \cref{appendix:anti-thrashing}.) 
The resource scaling tests presented in \cref{subsubsec:strong-scaling} illustrate how performance improves as more resources are allocated to {\proj}, thereby providing insight into how {\proj} would perform with nearly unbounded resources.

%The objective of our experimental evaluation of {\proj}, was to answer the following questions:
Our evaluation aims to answer the following questions:
\begin{itemize}
    \item How does {\proj} scale for individual DFS operations (\cref{subsec:eval-scaling})? 
    \item To what extent does FaaS' auto-scaling improve performance, scalability, and resource efficiency (\cref{subsec:eval-scaling}, \cref{subsec:real-world-workload})? 
    \item How does {\proj} perform under industrial workloads (\cref{subsec:real-world-workload})?
    \item How much does FaaS-based {\proj} cost (\cref{subsubsec:real-world-cost})?
    %compared to a serverful MDS (\cref{subsubsec:real-world-cost})?
    %\item How does the pay-per-use cost model of FaaS impact {\proj}'s cost (\cref{subsubsec:real-world-cost})?
    \item Can \proj benefit other DFSes besides HopsFS (\cref{sec:indexfs-results})? 
    \item \addcomment{How does the performance of {\proj} compare to other large-scale DFSes (\cref{subsec:eval-scaling})?}
\end{itemize} 

\vspace{-4pt}
\subsection{Scalability}
\label{subsec:eval-scaling}
\vspace{-6pt}

\begin{figure*}[t]
%\vspace{-5pt}
\begin{center}
\includegraphics[width=1.0\textwidth]{graphs/weak_scaling/weak_scaling_combined_latest.pdf}
\vspace{-15pt}
\caption{\textit{Client-driven} scaling comparison between \diffcomment{the various systems}{{\proj} and HopsFS}. The total amount of vCPUs allocated to {\proj} and HopsFS was held constant at 512 vCPUs, and each client performed \diffcomment{3,072}{2,048} operations. The number of clients ranged from 8 to 1,024. \addcomment{Note that the $y$-axis for the {\texttt{\small{create}}} operation is log-scale.}}
\label{fig:weak_scale_throughput}
\vspace{-12pt}
\end{center}
\end{figure*}

%\subsubsection{Elastic Scaling}
In this section, we evaluate the scalability of {\proj}, HopsFS, \addcomment{HopsFS+Cache, InfiniCache, and CephFS} using two micro-benchmarks covering
%, each of which covers 
key DFS operations including \texttt{\small{read file}}, \texttt{\small{stat file}}, \texttt{\small{list dir}}, \texttt{\small{mkdir}}, and \texttt{\small{create file}}. 
%\added{
The first microbenchmark tests {\proj}' \textit{client-driven scaling}: the ability of {\proj} to automatically
%and vertically 
scale-out as the number of clients increases, given a fixed resource cap.
%or what we call \emph{vertical elasticity}, 
%where each individual serverless NameNode function deployment can elastically scale-up given a fixed resource cap. 
The second microbenchmark, which we call
%refer to as 
\textit{resource scaling}, tests horizontal scalability (i.e., performance scaling with more deployments) and intra-deployment, vertical auto-scaling. 
%Through these tests, {\proj} demonstrates its horizontal scalability \textit{and} vertical elasticity through intra-deployment auto-scaling. 
%To that end, t
The results of these tests illustrate {\proj}' ability to transparently adapt to increases in both request load and available resources in order to maximize performance.
%} 
%\textcolor{red}{
We allocated a maximum of 512 vCPUs to \diffcomment{all}{both} systems during these tests, and {\proj} provisioned at-most \diffcomment{76}{81} NameNodes, each with 5 vCPUs, meaning it only required at-most \diffcomment{$76 \times 6.25$ $=475/512$ (92.77\%)}{$81 \times 5$ $=405/512$ (79\%)} of its allocated vCPUs during these tests. 
%}
%The micro-benchmarks are driven by an open source application we developed to evaluate the two frameworks.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Strong Scaling Throughput Figure %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
%\vspace{-5pt}
\begin{center}
\includegraphics[width=1.0\textwidth]{graphs/strong_scaling/strong_scaling_combined_latest.pdf}
\vspace{-14.5pt}
\caption{\textit{Resource scaling} comparison between \diffcomment{the various systems}{{\proj} and HopsFS}. The total amount of vCPUs allocated to \diffcomment{the systems}{{\proj} and HopsFS} ranged from 16 \diffcomment{to}{and} 512. \addcomment{For each problem size}, both systems used the same number of clients, each of which performed \diffcomment{3,072}{2,048} operations. \delcomment{Figure~\ref{fig:auto-scaling} shows a comparison of {\proj}' performance with and without auto-scaling (``AS'') enabled.}}
\label{fig:strong_scale_throughput}
\vspace{-13pt}
\end{center}
\end{figure*}
% \begin{figure*}[t]
% %\vspace{-5pt}
% \begin{center}

% \subfigure[Read file.] {
% \includegraphics[width=0.195\textwidth]{graphs/strong_scaling/strong_read.pdf}
% \label{fig:l_ss_read}
% }
% \hspace{-12pt}
% \subfigure[Stat file.] {
% \includegraphics[width=0.195\textwidth]{graphs/strong_scaling/strong_stat.pdf}
% \label{fig:l_ss_stat}
% }
% \hspace{-12pt}
% \subfigure[List directory.] {
% \includegraphics[width=0.195\textwidth]{graphs/strong_scaling/strong_ls.pdf}
% \label{fig:l_ss_ls_dir}
% }
% \hspace{-12pt}
% \subfigure[Create file.] {
% \includegraphics[width=0.195\textwidth]{graphs/strong_scaling/strong_create.pdf}
% \label{fig:l_ss_create_file}
% }
% \hspace{-12pt}
% \subfigure[Create directory.] {
% \includegraphics[width=0.195\textwidth]{graphs/strong_scaling/strong_mkdir.pdf}
% \label{fig:l_ss_mkdir}
% }
% % \hspace{-12pt}
% % \subfigure[Auto-scaling.] {
% % \includegraphics[width=0.195\textwidth]{graphs/autoscaling/autoscaling_latest.pdf}
% % \label{fig:auto-scaling}
% % }
% \vspace{-10pt}
% \caption{\textit{Resource scaling} comparison between \diffcomment{the various systems}{{\proj} and HopsFS}. The total amount of vCPUs allocated to {\proj} and HopsFS ranged from 16 and 512. \addcomment{For each problem size}, both systems used the same number of clients, each of which performed \diffcomment{3,072}{2,048} operations. Figure~\ref{fig:auto-scaling} shows a comparison of {\proj}' performance with and without auto-scaling (``AS'') enabled.}
% \label{fig:strong_scale_throughput}
% \vspace{-12pt}
% \end{center}
% \end{figure*}


%\subsubsection{Weak Scaling}
\subsubsection{Client-Driven Scaling}
\label{subsubsec:weak-scaling}
%For the client-driven scaling experiments, 
In this test, the amount of vCPUs allocated to both frameworks was fixed at 512 vCPUs to maximize performance, and each individual client executed \diffcomment{3,072}{2,048} file system operations. The total number of clients configured for each framework was varied between 8 and 1,024 in order to provide a wide range of scales to evaluate the frameworks. The results of this experiment are shown in Figure~\ref{fig:weak_scale_throughput} for throughput. (For latency results from this test, see Figure~\ref{fig:weak_scale_latency_cdf} in the Appendix.)
%and latency, respectively. 
%

{\proj} \addcomment{ultimately} achieves higher throughput for all read operations (i.e., \texttt{\small{read file}}, \texttt{\small{stat file}}, \texttt{\small{list dir}}) for all problem sizes:   
%For read-based operations,
{\proj} averaged 
%2067.36\% 
\diffcomment{$28.91\times$}{$21.67\times$},
%544.39\% 
\diffcomment{$8.22\times$}{$6.44\times$}, and 
%262.54\% 
\diffcomment{$20.53\times$}{$3.62\times$} higher throughput than HopsFS for \texttt{\small{read file}}, \texttt{\small{stat file}}, and \texttt{\small{list dir}}, respectively. \added{CephFS outperforms the other file systems for \texttt{\small{read file}} and \texttt{\small{stat file}} for up to and including 128 clients but fails to scale well beyond this point, only outperforming HopsFS and \textsc{InfiniCache}. {\proj} outperforms HopsFS+Cache for \texttt{\small{read file}} and \texttt{\small{list dir}} and achieves comparable performance for \texttt{\small{stat file}}.} 
%In the case of \texttt{\small{stat file}}, {\proj}'s throughput averages %544.39\% (
%$6.44\times$ higher than HopsFS with 1,024 clients. Finally, {\proj} achieves 262.53\% ($3.62\times$) higher throughput compared to HopsFS for 1,024 clients performing \texttt{\small{ls dir}} operations. 

There are several reasons for the throughput differences.
%achieved by the two systems. 
First, {\proj}' elastic caching layer efficiently serves metadata to clients from the memory of serverless functions
%the main memory of the serverless functions 
rather than from the persistent metadata store that is two network hops away. This also decreases the likelihood of the persistent metadata store becoming a bottleneck,
%that the persistent metadata store will become a bottleneck, 
as it is with HopsFS. 
Second, {\proj} is able to elastically scale-out its function deployments to satisfy the increasing request load, whereas HopsFS is limited by its fixed-scale deployment. For example, under {\proj}, there were 20 active NameNode instances for the 8 client case \addcomment{during the \texttt{\small{read file}} test}, and this transparently scaled-out to \diffcomment{74}{81} NameNodes for the 1,024 client case. This illustrates the necessity of using FaaS in the design of {\proj}, as FaaS offers
%provides rapid and elastic 
auto-scaling. 
%\added{

\diffcomment{It is also worth noting that {\proj} used at-most 462.5, 425, and 475 of the 512 available vCPU during the \texttt{\small{read}}, \texttt{\small{ls}}, and \texttt{\small{stat}} client-driven scaling tests, respectively.}{It is also worth noting that {\proj} used at-most \diffcomment{475/512}{405/512} vCPUs during the client-driven scaling tests, often using closer to 300-350 vCPUs.} This illustrates {\proj}' resource efficiency, as {\proj} can achieve strong performance with a fraction of the available resources.
%}

The throughput achieved during the \texttt{\small{list dir}} tests decreases for the last two problem sizes, unlike \texttt{\small{read file}} and \texttt{\small{stat file}}. This is likely because  \texttt{\small{list dir}} generates more garbage-collected intermediate data than \texttt{\small{read file}} and \texttt{\small{stat file}}. Because serverless functions have limited memory, this can degrade performance more noticeably than it would with large, serverful NameNodes. This problem can be mitigated by simply increasing the memory size for the serverless functions.
%that host the NameNode. 
%\added{We were unable to do this, as higher-memory instance types were unavailable to us when we conducted our experiments.}

For \texttt{\small{create file}} and \texttt{\small{mkdir}}, the performance disparity between {\proj} and HopsFS was not as significant as it was with read-based operations. The magnitude of the throughput achieved by both systems is also considerably lower than that of
%\added{that which} was achieved for 
read operations. Specifically, {\proj} achieved 49.09\% (1.49$\times$) higher throughput than HopsFS for \texttt{\small{create file}}. For \texttt{\small{mkdir}}, the two systems achieved roughly the same throughput. The reason both systems achieved significantly lower throughput for write operations is because the persistent metadata store quickly becomes a bottleneck. \addcomment{\textsc{InfiniCache} experienced poor performance for similar reasons as with the \texttt{\small{read}} operations. HopsFS+Cache also experienced low throughput \bencomment{Why?}. CephFS achieved significantly higher throughput than the other frameworks \bencomment{Why?}.}

%\subsubsection{Strong Scaling}
\subsubsection{Resource Scaling}
\label{subsubsec:strong-scaling}
For the resource scaling experiments, the total amount of vCPUs allocated to each framework was varied between 16 and 512. 
%\added{
As such, this experiment helps to elucidate how {\proj} would scale both horizontally and vertically with nearly unbounded (or at least additional) resources. Note that
%} 
for each vCPU value, all systems used the same amount of clients, each of which performed \diffcomment{3,072}{2,048} operations. The largest throughput obtained is reported.

Figure~\ref{fig:strong_scale_throughput} shows the results.
%of the strong scaling experiments. 
For read operations (\texttt{\small{read file}}, \texttt{\small{stat file}}, and \texttt{\small{list dir}}), {\proj} exhibits significantly better scaling behavior than \added{HopsFS, \textsc{InfiniCache}, and CephFS,} with 
%achieving significantly 
higher throughput as the resources scale. 
For the largest problem size, {\proj} achieves 
\diffcomment{$30.67\times$}{$16.50\times$}, 
\diffcomment{$9.30\times$}{$5.54\times$}, and 
\diffcomment{$20.69\times$}{$4.96\times$} higher throughput than HopsFS for \texttt{\small{read file}}, \texttt{\small{stat file}}, and \texttt{\small{list dir}}, respectively. Likewise, {\proj}' throughput increases by %2,424.42\%, 2,562.46\%, and 2,558.14\% for %\texttt{\small{read file}}, \texttt{\small{stat file}}, and \texttt{\small{list dir}}, 
\diffcomment{$34.60\times$}{$24.24\times$}, 
\diffcomment{$34.80\times$}{$25.62\times$}, and 
\diffcomment{$72.08\times$}{$25.58\times$}
for the same operations when scaling the number of vCPUs from 16 to 512. This is because allocating more resources to {\proj} enables a higher degree of auto-scaling. For smaller vCPU allocations, {\proj}' auto-scaling is limited and it cannot dynamically adapt to the workload, resulting in worse performance. 
%Note that t
The performance trend is less dramatic for write operations since the persistent metadata store is the bottleneck.

%for the largest problem size, respectively. 
%For \texttt{\small{read file}} operations, {\proj} achieves 
%1,550.2\% 
%16.50$\times$ higher throughput compared to HopsFS with 512 vCPUs. For \texttt{\small{stat file}} operations, {\proj} achieved 454.36\% ($5.54\times$) greater throughput than HopsFS for the largest problem size. Finally, {\proj} achieved 369.867\% (or $4.69\times$) higher throughput compared to HopsFS for \texttt{\small{ls dir}} operations with 512 vCPU. 

% Yue: NNs, each configured with 200 RPC handler threads, are not able to fully utilize the allocated resources as they are simply forwarding requests and responses between clients and backend NDB cluster. Therefore, even though NNs have thousands of threads they perform poorly with a low resource utilization. Configuring more number of stateless NNs help but the NN deployment scale can only be determined offline and manually.
{\proj}' superior scaling behavior can once again be attributed to its metadata cache and its agile auto-scaling scheme. 
%provided by FaaS. 
%In particular, 
As the total amount of vCPUs increases, {\proj} provisions an increasingly large pool of concurrently-running serverless NameNodes. By using a large pool of relatively ``small'' serverless NameNodes, {\proj} achieves high resource utilization, as each individual NameNode instance utilizes a majority of its allocated resources. This in turn enables {\proj} to achieve high performance with relatively modest resource allocations.  
%\added{

Though each HopsFS NameNode was configured with 200 RPC handler threads, HopsFS was not able to fully utilize the allocated resources, because its stateless NameNodes essentially serve as proxies, forwarding requests/responses between clients and the metadata store. This also explains why HopsFS' NameNodes had a consistently low CPU utilization at around 70\%. Configuring more NameNode servers may help, but again, it is difficult to pre-determine how many NameNodes to deploy for optimal performance and resource utilization.
%the deployment scale required to achieve optimal performance with optimal resource consumption.
%}

\begin{figure}[h]
    \centering
    \vspace{-12pt}
    \includegraphics[width=0.35\textwidth]{graphs/autoscaling/autoscaling_latest.pdf}
    \vspace{-4pt}
    \caption{
    Performance comparison for {\proj} with full, limited, and no auto-scaling.
        %Impact of enabling or disabling horizontal, intra-deployment auto-scaling on throughput for {\proj}. With auto-scaling ``enabled'', individual deployments were free to scale-out as they did in the other experiments. With limited auto-scaling, deployments could scale-out to at most 2-3 \diffcomment{active}{concurrently-running} instances. With auto-scaling disabled, each deployment was limited to at-most one active NameNode instance.
    }
    \vspace{-12pt}
    \label{fig:auto-scaling}
\end{figure}

%\added{
%\delcomment{As shown in Figure~\ref{fig:auto-scaling}, {\proj} achieved \delcomment{$2.54\times$ and} $4.03\times$, \addcomment{$3.64\times$, and $3.10\times$} higher throughput for \texttt{\small{read}}, \texttt{\small{stat}}, and \texttt{\small{ls}} operations with auto-scaling enabled compared to %limited and 
%disabled auto-scaling, \addcomment{respectively}. %, respectively. 
%This demonstrates the strong performance benefit of {\proj}' auto-scaling.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This paragraph was previously the caption of the fig:auto-scaling figures. %
% It takes up less  space as a proper paragraph, however.                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addcomment{Figure~\ref{fig:auto-scaling} shows the impact on system throughput of enabling or disabling horizontal, intra-deployment auto-scaling for {\proj} across various file system operations. With auto-scaling ``enabled'', individual deployments were free to scale-out as they did in the other experiments. With limited auto-scaling, deployments could scale-out to at most 2-3 \diffcomment{active}{concurrently-running} instances. With auto-scaling disabled, each deployment was limited to at-most one active NameNode instance.}

\diffcomment{{\proj} achieved between $2.85 - 3.17\times$ and $3.53 - 3.80\times$ higher throughput for \texttt{\small{read}} and \texttt{\small{stat file}} operations with auto-scaling enabled compared to limited and disabled auto-scaling, respectively. This trend is even more pronounced for \texttt{\small{ls}}, with {\proj} observing $3.07\times$ and $14.37\times$ higher throughput with auto-scaling enabled compared to limited and disabled auto-scaling, respectively. The difference is less severe for write operations (i.e., \texttt{\small{create file}} and \texttt{\small{mkdir}}), as the bottleneck for writes is the persistent metadata store. These results illustrate the importance of FaaS-enabled elastic auto-scaling within {\proj}'s design as well as its significant impact on {\proj}' performance.}{{\proj} achieved \diffcomment{$3.17\times$}{$2.54\times$} and \diffcomment{$3.80\times$}{$4.03\times$} higher throughput for \texttt{\small{read file}} operations with auto-scaling enabled compared to limited and disabled auto-scaling, respectively. This trend continues for \texttt{\small{stat file}} operations, with auto-scaling enabling approximately \diffcomment{$2.85\times$}{$2.24\times$} and \diffcomment{$3.53\times$}{$3.81\times$} higher throughput compared to limited and disabled auto-scaling, respectively. The difference is less severe for write operations (i.e., \texttt{\small{create file}} and \texttt{\small{mkdir}}), as the bottleneck for writes is the persistent metadata store. This demonstrates the strong performance benefit of {\proj}' auto-scaling.}

%{\proj} achieved \diffcomment{$3.17\times$}{$2.54\times$} and \diffcomment{$3.80\times$}{$4.03\times$} higher throughput for \texttt{\small{read file}} operations with auto-scaling enabled compared to limited and disabled auto-scaling, respectively. This trend continues for \texttt{\small{stat file}} operations, with auto-scaling enabling approximately \diffcomment{$2.85\times$}{$2.24\times$} and \diffcomment{$3.53\times$}{$3.81\times$} higher throughput compared to limited and disabled auto-scaling, respectively. The difference is less severe for write operations (i.e., \texttt{\small{create file}} and \texttt{\small{mkdir}}), as the bottleneck for writes is the persistent metadata store. \diffcomment{These results illustrate the importance of FaaS-enabled elastic auto-scaling within {\proj}'s design as well as its significant impact on {\proj}' performance.}{This demonstrates the strong performance benefit of {\proj}' auto-scaling.}

%%%%%%%%%%%%%%%%%
% Commented-Out %
%%%%%%%%%%%%%%%%%
\if 0 % yue: above sentence is the shortened version of the paragraph shown as below:
Figure~\ref{fig:autoscaling} shows the impact on system throughput of enabling or disabling horizontal, intra-deployment auto-scaling for {\proj} across various file system operations during the client-driven scaling tests. 
%With auto-scaling ``enabled'', individual deployments were free to scale-out as they did in the other experiments. With limited auto-scaling, deployments could scale-out to at most 2-3 concurrently-running instances. Finally, with auto-scaling disabled, each deployment was limited to at-most one active NameNode instance. 
%
{\proj} achieved 
%145.60\% 
$2.45\times$ 
and 
%310.86\% 
$4.10\times$ higher throughput for \texttt{\small{read file}} operations with auto-scaling enabled compared to limited and disabled auto-scaling, respectively. This trend continues for \texttt{\small{stat file}} operations, with auto-scaling enabling approximately
%124.70\% 
$2.24\times$ and 
%281.81\% 
$3.81\times$ higher throughput compared to limited and disabled auto-scaling, respectively. The result for \texttt{\small{list dir}} was similar. The difference is less severe for write operations (i.e., \texttt{\small{create file}} and \texttt{\small{mkdir}}), as the bottleneck for writes is the persistent metadata store. 
\fi 
%We evaluate the performance benefits of {\proj}' auto-scaling in \cref{subsubsec:autoscaling}.  

% \if 0 % yue: used subfigure instead
% \begin{figure}[t]
% %\vspace{-12pt}
% \centering
% \begin{minipage}{\textwidth}

% \begin{minipage}[b]{0.232\textwidth}
% \begin{center}
% \includegraphics[width=1\textwidth]{graphs/latency_cdfs/weak_scale_latency_cdf_full_v3.pdf}
% \end{center}
% \vspace{-12pt}
% \subcaptionbox{
% Full figure.
% }
% \label{fig:weak_scale_latency_cdf_full}
% \end{minipage}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\hfill
% %\hspace{1em}%
% %\hspace{4pt}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{minipage}[b]{0.236\textwidth}
% \begin{center}
% \includegraphics[width=1\textwidth]{graphs/latency_cdfs/weak_scale_latency_cdf_zoomed_v3.pdf}
% \end{center}
% \vspace{-12pt}
% \subcaptionbox{
% Zoomed-in.
% }
% \label{fig:weak_scale_latency_cdf_zoomed}
% \end{minipage}

% \end{minipage}
% \vspace{-8pt}
% \caption{Latency CDF for various file system operations at roughly 50\% capacity for both {\proj} and HopsFS.}
% \vspace{-2pt}
% \label{fig:weak_scale_latency_cdf}
% \end{figure}
% \fi 


\subsubsection{Subtree Operations}

\begin{wraptable}{r}{0.52\columnwidth}
\vspace{-16pt}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Subtree Op Latency Table %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\scalebox{0.95}{
%\begin{table}[htbp]
\centering
\caption{Average end-to-end latency (ms) of subtree {\texttt{\small{mv}}} operations for varying directory sizes.}
\vspace{-2pt}
\scalebox{0.8}{
\begin{tabular}{@{}lrl@{}}
%\toprule
\Xhline{2\arrayrulewidth}
\textbf{Directory Size} & \multicolumn{1}{r}{\textbf{HopsFS}} & \multicolumn{1}{r}{\textbf{$\lambda$MDS}}          \\ %\midrule
\hline
262k ($2^{18}$)         & 7,511.60                            & \multicolumn{1}{r}{6,455.80}  \\
524k ($2^{19}$)         & 14,184.80                           & \multicolumn{1}{r}{12,509.20} \\ 
1.04M ($2^{20}$)        & 25,137.00                           & 25,220.80                     \\ 
%\bottomrule
\hline
\end{tabular}
} % end of scalebox
\vspace{-12pt}
\label{tab:subtree-mv}
%\end{table}
\end{wraptable}

Table~\ref{tab:subtree-mv} shows the end-to-end latency of a \texttt{\small{mv}} operation performed on directories containing a large number of files. We varied the directory size between $2^{18}$ and $2^{20}$. On average, {\proj} completed the \texttt{\small{mv}} operation in 
%approximately 
16.35\% less time than HopsFS for the $2^{18}$-file directory. For $2^{19}$-file directories, {\proj} was about 13.39\% faster. Finally, for $2^{20}$-file directories, the two frameworks achieved roughly the same end-to-end latency. For large subtree operations, the persistent metadata store quickly becomes the bottleneck, as every write operation must update the persistent state in the database. 
%This is particularly true for \texttt{\small{delete}} operations, which modify every single node within a subtree, unlike \texttt{\small{mv}}. \bencomment{Not sure what to say here, as the \texttt{\small{delete}} results were poor and are being omitted...}


\vspace{-4pt}
\subsection{Industrial Workload}
\label{subsec:real-world-workload}
\vspace{-6pt}

In this section, we present and discuss the results of executing a real-world, industrial workload on both {\proj} and HopsFS. The workload we use is based on the one used in HopsFS' evaluation, which was generated using statistics from traces of Spotify's 1600-node HDFS cluster. The frequencies of the file system operations are shown in Table~\ref{tab:spotify-operation-percentages}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spotify Operation Percentages Table %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\vspace{-6pt}
\caption{Relative frequency of the file system operations used in the Spotify workload experiment.}
\vspace{-6pt}
\resizebox{0.475\textwidth}{!}{
\begin{tabular}{@{}lr|lr@{}}
\rowcolor[HTML]{d6eaf8} 
\textbf{Operation} & \textbf{Percentage} & \textbf{Operation}                & \textbf{Percentage}             \\
create file & 2.7\%  & read file     & 69.22\% \\
\rowcolor[HTML]{EFEFEF} 
mkdirs      & 0.02\% & stat file/dir & 17\%    \\
delete file/dir  & 0.75\% & list file/dir & 9.01\%  \\
\rowcolor[HTML]{EFEFEF} 
mv file/dir             & 1.3\%               & \cellcolor[HTML]{9AFF99}\textbf{Total Read Ops} & \cellcolor[HTML]{9AFF99}\textbf{95.23\%}
\end{tabular}}
\label{tab:spotify-operation-percentages}
%\vspace{-3pt}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spotify Throughput Comparison + Perf-per-Cost Figure %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}
%     \centering
%     \includegraphics[width=1\textwidth]{graphs/spotify/spotify_row_chart.pdf}
%     \vspace{-14pt}
%     \caption{The left and middle plots show a throughput comparison during the two Spotify workloads. The number of active {\proj} NameNodes (``NNs'') is shown on the secondary $y$-axis. ``CN'' means ``cost-normalized''. The right plot shows a performance-per-cost comparison between {\proj} and HopsFS+Cache for both versions of the Spotify workload.
%     }
%     \label{fig:spotify-throughput-and-perf-per-cost}
% \end{figure*}

\begin{figure*}[t]
%\vspace{-5pt}
\begin{center}
\subfigure[Base: 25,000 ops/sec.] {
\includegraphics[height=0.177125\textheight]{graphs/spotify/spotify_25k_latest.pdf}
\label{fig:spotify-25k-throughput-new}
}
\hspace{-8pt}
\subfigure[Base: 50,000 ops/sec] {
\includegraphics[height=0.177125\textheight]{graphs/spotify/spotify_50k_latest.pdf}
\label{fig:spotify-50k-throughput-new}
}
\hspace{-8pt}
\subfigure[Performance-per-cost comparison.] {
\includegraphics[height=0.177125\textheight]{graphs/spotify/spotify_25k_50k_perf_per_cost_latest.pdf}
\label{fig:spotify-perf-per-cost-new}
}
\vspace{-8pt}
\caption{Throughput and performance-per-cost comparison between \diffcomment{the various frameworks}{{\proj} and HopsFS} during the Spotify workload.
The number of active {\proj} NameNodes (``NNs'') is shown on the secondary $y$-axis in the left and middle sub-plots.}
\label{fig:spotify-throughput-and-perf}
\vspace{-14pt}
\end{center}
\end{figure*}

% \begin{figure}[t]
% %\vspace{-5pt}
% \begin{center}
% \subfigure[Base: 25,000 ops/sec.] {
% \includegraphics[width=0.25\textwidth]{graphs/spotify/spotify_25k_latest_thin.pdf}
% \label{fig:spotify-25k-throughput-new}
% }
% \hspace{-10pt}
% \subfigure[Base: 50,000 ops/sec] {
% \includegraphics[width=0.195\textwidth]{graphs/spotify/spotify_50k_latest_thin.pdf}
% \label{fig:spotify-50k-throughput-new}
% }
% \vspace{-8pt}
% \caption{Throughput comparison between \diffcomment{the various frameworks}{{\proj} and HopsFS} during the Spotify workload.
% The number of active {\proj} NameNodes (``NNs'') is shown on the secondary $y$-axis.}
% \label{fig:spotify-throughput}
% \vspace{-14pt}
% \end{center}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spotify 25k and 50k side-by-side throughput chart %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[width=0.485\textwidth]{graphs/spotify/spotify_25k_50k_latest.pdf}
%     \vspace{-14pt}
%     \caption{Throughput comparison during the two Spotify workloads. The number of active {\proj} NameNodes (``NNs'') is shown on the secondary $y$-axis. ``CN'' means ``cost-normalized''. 
%     }
%     \label{fig:spotify-25k-50k-throughput-new}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.485\textwidth]{graphs/spotify/spotify_25k_latest.pdf}
%     \vspace{-14pt}
%     \caption{Throughput comparison during the Spotify workload with a base throughput of 25,000 ops/sec. The number of active {\proj} NameNodes (``NNs'') is shown on the secondary $y$-axis.}
%     \label{fig:spotify-25k-throughput-new}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.485\textwidth]{graphs/spotify/spotify_50k_latest.pdf}
%     \vspace{-14pt}
%     \caption{Throughput comparison during the Spotify workload with a base throughput of 50,000 ops/sec. The number of active {\proj} NameNodes (``NNs'') is shown on the secondary $y$-axis.}
%     \label{fig:spotify-50k-throughput-new}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spotify Latency Comparison Figures %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
%\vspace{-5pt}
\begin{center}
\includegraphics[width=1.0\textwidth]{graphs/spotify/latency_cdf.pdf}
% \subfigure[Base throughput: 25,000 ops/sec.] {
% \includegraphics[width=.975\textwidth]{graphs/spotify/Spotify_25kLOC_LatencyCDF.pdf}
% \label{fig:spotify-25k-latency-cdf}
% }
% \subfigure[Base throughput: 50,000 ops/sec] {
% \includegraphics[width=.975\textwidth]{graphs/spotify/Spotify_50kLOC_LatencyCDF.pdf}
% \label{fig:spotify-50k-latency-cdf}
% }
\vspace{-16pt}
\caption{Latency CDF comparison between \diffcomment{{\proj} (``$\lambda$''), HopsFS (``H''), and HopsFS+Cache (``H+C'')}{(``$\lambda$'') and HopsFS (``H'')} for \diffcomment{both}{the two} versions of the Spotify workload.}
\label{fig:spotify-latency-cdf}
\vspace{-10pt}
\end{center}
\end{figure*}

%\subsubsection{Experimental Setup \& Configuration}
\subsubsection{Experimental Setup}
%To drive the workload, we use a modified version of the \texttt{\small{hammer-bench}} utility used to conduct HopsFS' evaluation~\cite{hopsfs_fast17, hammer-bench}. 
%To drive this experiment, 
We implemented a DFS benchmark that can generate bursty file system loads by modifying the \texttt{\small{hammer-bench}} utility used to conduct HopsFS' evaluation~\cite{hammer-bench, hopsfs_fast17}.
Our benchmark randomly varies system throughput over the course of the workload's execution in order to accurately simulate a real-world DFS workload~\cite{igen_cloud16}. Specifically, our benchmark executes the workload for 5~minutes. Every 15~seconds, the benchmark generates a random throughput value $\Delta$ from a Pareto distribution with a shape parameter $\alpha=2$. (Please refer to~\cite{igen_cloud16} for a discussion on why the Pareto distribution is useful in this scenario.) Let $n$ be the number of client VMs used in the experiment. Each client VM will attempt to sustain $\delta = \frac{\Delta}{n}$ ops/sec. If less than $\delta$ operations are completed during a given second, then the remaining operations roll over to the next second. 

In order to demonstrate {\proj}' ability to elastically scale in response to bursts of metadata requests, the benchmark randomly generates throughput spikes up to $7\times$ greater than the \emph{base} throughput. We ran two different versions of the workload: one in which the Pareto distribution's scale parameter $x_t=25,000$ and the other in which $x_t=50,000$. The value of $x_t$ determines the base throughput of the workload. 



%\textcolor{red}{
Both workloads were executed by 1,024 clients across 8 VMs. We allocated 512 vCPUs to HopsFS in order to maximize its performance during these tests. While allocating less vCPUs would've been cheaper, HopsFS' performance would've suffered, as illustrated by the resource scaling tests.
%} 
%\added{
Each \textit{individual} {\proj} NameNode is allocated 5 vCPUs, and in the 25,000 ops/sec workload, {\proj}' NameNode cluster is collectively allocated just 50\% of the total vCPU resources allocated to HopsFS' NameNode cluster in order to better illustrate {\proj}' resource and cost efficiency.
%}

\subsubsection{Throughput \& Latency}
%Figure~\ref{fig:spotify-25k-throughput-new} 
\addcomment{Figure~\ref{fig:spotify-25k-throughput-new}} shows a throughput comparison between {\proj} and HopsFS during an execution of the Spotify workload with a base throughput of 25,000~ops/sec. Note that each of {\proj}' NameNodes was configured with 6GB of RAM for the 25,000 ops/sec workload. {\proj} achieved an average throughput of 45,690.34~ops/sec and an average latency of 1.02~ms
%1.0156~ms 
during the execution of this workload. HopsFS achieved an average throughput of 38,134.35~ops/sec and an average latency of 10.58~ms. %\added{Notably, {\proj}'s NameNodes were allocated only 50\% of the vCPU allocated to HopsFS' NameNodes (256 vCPUs vs. 512 vCPUs, respectively) for this experiment, and {\proj} ultimately used only 155/256 of its allocated vCPUs to complete the workload.}

%\added{
Summarily, {\proj} achieved 90.40\% (10.41$\times$) lower latency and 16.53\% (1.19$\times$) higher throughput on average than HopsFS, while using 39.45\% less resources.
%} 
{\proj} was able to fully sustain the entire workload, including the entire 15-second 163,996~ops/sec burst generated around time $t=200$. Meanwhile, HopsFS' clients struggled to sustain loads above 38,000~ops/sec. When the burst occurred, HopsFS had already ``fallen behind'' and was struggling to execute operations that had been generated nearly a minute prior. So, {\proj}' peak sustained, throughput was 
%330.04\% (
4.3$\times$
higher than that of HopsFS.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.475\textwidth]{graphs/spotify/Spotify_50kLOC_Throughput.pdf}
%     \vspace{-24pt}
%     \caption{Throughput comparison between {\proj} and HopsFS during an execution of the Spotify workload with a base throughput of 50,000 ops/sec.}
%     \vspace{-18pt}
%     \label{fig:spotify-50k-throughput}
% \end{figure}


Figure~\ref{fig:spotify-50k-throughput-new} shows a throughput comparison 
%between {\proj} and HopsFS 
during an execution of the Spotify workload with a base throughput of 50,000~ops/sec. For this test, {\proj}' NameNode cluster was allocated a full 512 vCPU but used at most 180/512 (35.15\%) of the available vCPUs. {\proj} achieved an average throughput of 90,875.60~ops/sec and an average latency of 4.31~ms during 
%the execution of 
this workload. HopsFS achieved an average throughput of 44,956.28~ops/sec and an average latency of 22.40~ms. 

HopsFS was unable to achieve the base throughput of 50,000~ops/sec, so it spent the duration of the workload attempting to ``catch up''. Meanwhile, {\proj} sustained approximately 250,000 ops/sec during the burst at around $t=200$. To this end, {\proj}' peak, sustained throughput was 456.09\% (5.56$\times$) higher than that of HopsFS.

{\proj}' average throughput was 102.14\% (2.02$\times$) greater than HopsFS'; similarly, {\proj}' average latency was 80.76\% (5.19$\times$) lower than HopsFS'. For ``read'' operations, {\proj} achieves an average latency anywhere from $6.93\times$-$20.13\times$ lower than that of HopsFS (see Figure~\ref{fig:spotify-latency-cdf}). However, {\proj} is unable to complete ``write'' operations as quickly as HopsFS because of the added overhead required by {\proj}' coherence protocol. Summarily, HopsFS achieves 1.5$\times$-$5.55\times$ shorter ``write'' latencies compared to {\proj}. 

\addcomment{\textsc{InfiniCache} failed to complete either of the two Spotify workloads. The FaaS platform became overwhelmed by the volume of HTTP requests. Likewise, the high-latency HTTP requests and static, fixed-size deployment were insufficient for both the base throughput and bursts of work during the workload.}

\addcomment{Because FaaS assumes a near-unbounded amount of sources, fixing the amount of vCPU allocated to the platform results in poor performance and scalability. To perform a fair comparison and highlight the cost-saving benefits of FaaS, we also compare {\proj} against a ``cost-normalized'' configuration of HopsFS+Cache, referred to as ``CN HopsFS+Cache''. 
Specifically, we configured CN HopsFS+Cache with $72$ and $144$ vCPU for the 25,000 and 50,000 ops/sec Spotify workloads, respectively. In doing so, CN HopsFS+Cache incurs the same monetary cost as {\proj}. Considering first the 25,000 ops/sec workload as shown in Figure~\ref{fig:spotify-25k-throughput-new},
%Figure~\ref{fig:spotify-25k-throughput-new}, 
CN HopsFS+Cache achieves lower throughput than {\proj}, failing to sustain the burst of requests around the 200th second of the workload. This phenomenon occurs again during the 50,000 ops/sec workload as shown in Figure~\ref{fig:spotify-50k-throughput-new}.} %Figure~\ref{fig:spotify-50k-throughput-new}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spotify 25k Cost Comparison Figure %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    %\vspace{-15pt}
    \centering
    \includegraphics[width=0.475\textwidth]{graphs/spotify/spotify_cumulative_cost.pdf}
    \vspace{-4pt}
    \caption{Cumulative cost of the 25k ops/sec Spotify workload. HopsFS' cost was \$2.50. {\proj}' cost was \$0.35 using AWS Lambda's prices, which are \$0.0000166667 per GB-second, charged at 1ms granularity, and \$0.20 per 1M requests~\cite{lambda_pricing}. %Using the hourly cost for Google Compute Engine \texttt{\small{c2-standard-16}} instances (\$0.9406 per hour~\cite{gce_vm_prices}), {\proj}'s cumulative cost was \$0.28.
    }
    \vspace{-4pt}
    \label{fig:spotify-25k-cost-cumulative}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.475\textwidth]{graphs/perf_per_cost/perf_per_cost.pdf}
    \vspace{-4pt}
    \caption{Performance-per-cost comparison between {\proj} and HopsFS+Cache for read-based file system operations.}
    \vspace{-5pt}
    \label{fig:perf-per-cost-client-driven}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.485\textwidth]{graphs/spotify/spotify_25k_50k_perf_per_cost.pdf}
%     \vspace{-15pt}
%     \caption{Performance-per-cost comparison between {\proj} and HopsFS+Cache for both versions of the Spotify workload.}
%     \label{fig:spotify-perf-per-cost-new}
%     \vspace{-6pt}
% \end{figure}

\subsubsection{In-Memory Metadata Cache}
To measure the performance impact of {\proj}' metadata caching layer, we executed a second instance of the $x_t=25,000$ workload in which we decreased the capacity of the serverless NameNode cache to less than half the working set size (WSS) of the workload. 
%The result of this execution is also shown in 
As shown in Figure~\ref{fig:spotify-25k-throughput-new}, %Figure~\ref{fig:spotify-25k-throughput-new}, 
{\proj} with a smaller cache still achieves better performance than HopsFS, sustaining between 70,000-80,000~ops/sec during the largest burst. Despite failing to sustain 164,000~ops/sec, \addcomment{reduced-cache} {\proj} \diffcomment{quickly caught up and completed}{was able to quickly catch up and complete} the remainder of the workload as generated.  

\subsubsection{Elastic Auto-Scaling}



\label{subsubsec:autoscaling}
The results of the Spotify workload demonstrate 
%\added{
{\proj}' ability to handle large bursts of work. 
%{\proj} takes advantage of the elastic auto-scaling provided by its FaaS platform to transparently scale-out additional NameNodes during bursts of request. 
%Figures~\ref{fig:spotify-25k-throughput-new} and~\ref{fig:spotify-50k-throughput-new} 
Figures~\ref{fig:spotify-25k-throughput-new} and~\ref{fig:spotify-50k-throughput-new} show that {\proj} immediately provisions additional NameNodes to satisfy the influx of requests from clients as soon as the workload starts. {\proj} quickly scales-out again around the 200-second mark, as this is when the 7$\times$ request burst occurs, demonstrating the effectiveness of {\proj}' auto-scaling policy. 
With unbounded resources, {\proj} could rapidly scale-out to much higher load spikes. \addcomment{This is further supported by the trend shown in the resource scaling experiments (Figure~\ref{fig:strong_scale_throughput}).}
%with a much higher peak-to-trough ratio.
%}



%%% yue: A better flow is to make this Monetary Cost subsubsection a subsection, separated away from the subsection Industrial Workload, as this subsection covers the cost efficiency for both scaling tests as well as Spotify tests. 
%\subsubsection{Monetary Cost}
\vspace{-2pt}
\subsection{Monetary Cost}
\vspace{-4pt}
\label{subsubsec:real-world-cost}
Figure~\ref{fig:spotify-25k-cost-cumulative} shows the cumulative cost during the 25,000~ops/sec Spotify workload for {\proj} and HopsFS. 
%\added{
For {\proj}, the cost is computed as follows: for every 1~ms interval of the workload, we bill each NameNode actively serving an HTTP or TCP request using AWS Lambda's prices (as described in Figure~\ref{fig:spotify-25k-cost-cumulative}). If no requests are actively being served by a particular NameNode, then that NameNode does not incur any cost. For HopsFS, we bill the cost of the entire 512-vCPU cluster for each 1~ms interval of the workload.
%} 
By the end of the workload, HopsFS' cumulative cost is \$2.50 while {\proj}' cumulative cost is just \$0.35. By taking advantage of FaaS' pay-per-use pricing model, {\proj} reduces the cost of executing the workload by 85.99\% (7.14$\times$) compared to HopsFS while achieving significantly better performance.

\addcomment{While the use of FaaS can yield improved elasticity, scalability, and performance, another primary benefits of FaaS is reduced tenant-side cost and increased cost-effectiveness. In particular, {\proj}' cost-effectiveness manifests via its ability to achieve superior or equivalent performance while using a smaller amount of resources. By saturating a large number of relatively small, individual serverless NameNodes, {\proj} exhibits high resource utilization and resource efficiency with respect to the resources provisioned to it by the FaaS provider. Likewise, by leveraging the pay-per-use property of FaaS, {\proj} is ultimately able to reduce workload costs while delivering equivalent or better performance.}

\addcomment{To quantify this notion of cost-efficiency, we define a new metric \textit{performance-per-cost}, which is given as one of $\frac{\text{instantaneous throughput}}{\text{instantaneous cost}}$ or $\frac{\text{instantaneous throughput}}{\text{total cost}}$. Therefore, the units of this metric are $\frac{operations/second}{\$} = \frac{operations}{second \times \$}$, or, operations per second per dollar. 
%$\frac{operations/second}{cost} = \frac{operations}{second \times cost}.$ 
The value of this metric is a measure of the cost-efficiency; a higher value indicates that the associated framework is able to achieve a higher performance-cost ratio, which is desirable. Increasing the value of this metric can be done using some combination of increasing throughput and decreasing cost.}

\addcomment{Figure~\ref{fig:perf-per-cost-client-driven} shows the average performance-per-cost for {\proj} and HopsFS+Cache for each problem size of the \textit{client-driven} scaling experiment. As with the real-world workload, the cost of HopsFS+Cache is computed as the cost of all 32 NameNode VMs running for the duration of the experiment; however, the cost of {\proj} was computed in a simplified manner. That is, the cost of each actively-running NameNode was billed for the duration of the experiment without determining whether or not actively serving requests for each unit of time (which ultimately inflates the reported cost of {\proj}).}

\addcomment{{\proj} achieved higher performance-per-cost values for both {\texttt{\small{read file}}} and {\texttt{\small{list dir}}} for all problem sizes. For {\texttt{\small{stat file}}}, {\proj} achieves higher performance-per-cost for eight problem sizes and roughly equivalent performance-per-cost for the others. {\proj} achieves higher performance-per-cost for {\texttt{\small{read file}}} because {\proj} achieved equivalent or higher throughput than HopsFS+Cache using a fraction of the resources; while HopsFS+Cache used 512 vCPU, {\proj} used at-most 475 vCPU by the largest problem size. This phenomenon occurred to an even greater degree for {\texttt{\small{list dir}}} for which {\proj} achieved $32.74$\% higher throughput with fewer resources. For {\texttt{\small{stat file}}}, {\proj} achieves equal or better cost-effectiveness compared to HopsFS+Cache, as the two frameworks achieved comparable performance, but {\proj} used fewer resources.}

\addcomment{Figure~\ref{fig:spotify-perf-per-cost-new} shows the performance-per-cost for each second of the real-world Spotify workload for {\proj} and HopsFS. The cost for HopsFS is computed as the cost of running the 32 NameNode VMs for one second, whereas the cost for {\proj} is calculated using the pay-per-use pricing model of FaaS. Specifically, the resources allocated to an active NameNode are only billed if that NameNode served a request within that second. {\proj} achieves significantly higher performance-per-cost compared to HopsFS+Cache. This is because {\proj} experiences near-equivalent or outright superior throughput compared to HopsFS+Cache for the entirety of the workload while using significantly fewer resources (at-most 180 vCPU for {\proj} compared to 512 vCPU for HopsFS+Cache).}




\vspace{-2pt}
\subsection{Fault Tolerance}
\vspace{-4pt}

\begin{figure}
    \centering
    \includegraphics[width=0.475\textwidth]{graphs/spotify/spotify_25k_failure_experiment.pdf}
    \vspace{-5pt}
    \caption{Results of the ``failure'' experiment using the 25,000 ops/sec Spotify workload.
    }
    \label{fig:spotify_25k_failure_test}
    \vspace{-5pt}
\end{figure}

\addcomment{In order to evaluate the fault tolerance mechanisms used by {\proj}, we execute another version of the 25,000 ops/sec Spotify workload in which we manually terminate a single active NameNode instance from each deployment in a round-robin fashion once every 30 seconds. When the workload began, {\proj} had already provisioned 36 NameNodes in order to ensure there were sufficient instances available for termination.}

\addcomment{The results of this experiment are shown in Figure~\ref{fig:spotify_25k_failure_test}. The darker dashed line shows the number of active {\proj} NameNodes over the course of the workload's execution. As shown in the figure, the number of active NameNodes decreasing by 1 every 30 seconds. When a failure occurs, {\proj} clients transparently and automatically resubmit TCP requests to other NameNode instances via TCP if there are any established connections available; otherwise, clients resubmit requests via HTTP. Failed HTTP requests are simply re-submitted via HTTP again. The results show that {\proj}'s throughput briefly destabilizes and decreases slightly when a failure occurs. This occurs because clients first block and wait for their requests to time-out, after which the requests are resubmitted.}

\addcomment{Despite periodic NameNode failures, {\proj} is able to sustain the sustain the workload's request load, even during the 164,000 ops/sec burst that occurred at around 200 seconds. Note that system throughput increases marginally shortly after termination events. This is because clients temporarily increase their request rate to ``make up'' for the drop in throughput that resulted from the termination event.}

%\added{rather than the number of NameNodes}.

% \begin{figure}[t]
%     \centering
%     \subfigure[Read file.] {
%     \includegraphics[width=0.235\textwidth]{graphs/latency_cdfs/weak_scale_latency_cdf_full.pdf}
%     \label{fig:l_ss_read}
%     }
%     \hspace{-8pt}
%     \subfigure[Stat file.] {
%     \includegraphics[width=0.235\textwidth]{graphs/latency_cdfs/weak_scale_latency_zoomed_most.pdf}
%     \label{fig:l_ss_stat}
%     }
%     %\includegraphics[width=0.475\textwidth]{graphs/latency_cdfs/weak_scale_latency_cdf_full.pdf}
%     %\vspace{-15pt}
%     \caption{Latency CDF for various file system operations at roughly 50\% capacity for both {\proj} and HopsFS.}
%     \label{fig:weak_scale_latency_cdf}
%     \vspace{-15pt}
% \end{figure}

\input{indexfs_result}

==> lessons.tex <==
% \vspace{-8pt}
\section{Lessons Learned}
\label{sec:lessons-learned}
\vspace{-4pt}

%While designing and implementing {\proj}, we learned several interesting lessons that have applicability beyond the scope of serverless metadata management. First of all, creating latency-sensitive applications atop FaaS requires techniques to mitigate the relatively high invocation overheads of serverless functions. Relying exclusively upon traditional HTTP-based invocations does not enable systems to achieve high throughput and low latency; instead, mechanisms such as {\proj}' TCP-RPC invocation method are necessary for achieving good performance. 

%Notably, introducing techniques to circumvent the large overhead associated with HTTP invocations can reduce the system's ability to harness the auto-scaling property of FaaS. Such techniques must be designed with care so as to carefully optimize the trade-off between maximizing performance and maximizing scalability. This can be considered an instance of the performance-parallelism trade-off --- a trade-off that has previously been observed in FaaS systems from other domains~\cite{wukong_socc20}. % To be clear, I am not recommending we cite Wukong in this paper. 

%The use of FaaS also introduces a number of relatively complicated error states. Serverless functions can be reclaimed by the cloud provider at any point. If TCP-RPC connections are dropped unexpectedly, re-establishing connections is non-trivial due to the lack of addressibility of serverless functions. Additionally, naively resubmitting erred tasks via HTTP can result in requests storms that overwhelm the serverless platform, leading to extreme over-provisioning of resources. This can ultimately cause a huge drop in performance and can cause errors elsewhere in the system --- for example, the persistent datastore may experience a temporary performance drop due to a wave of new connections from newly-provisioned NameNodes. To address this, FaaS-based systems must develop clever techniques to provide fault tolerance that do not trigger the aforementioned problems. 

==> tex_figures/strong_scaling.tex <==
\begin{figure*}[t]
%\vspace{-5pt}
\begin{center}

\subfigure[Read file.] {
\includegraphics[width=0.19\textwidth]{graphs/strong_scaling/strong_read.pdf}
\label{fig:l_ss_read}
}
\hspace{-8pt}
\subfigure[Stat file.] {
\includegraphics[width=0.19\textwidth]{graphs/strong_scaling/strong_stat.pdf}
\label{fig:l_ss_stat}
}
\hspace{-8pt}
\subfigure[List directory.] {
\includegraphics[width=0.19\textwidth]{graphs/strong_scaling/strong_ls.pdf}
\label{fig:l_ss_ls_dir}
}
\hspace{-8pt}
\subfigure[Create file.] {
\includegraphics[width=0.19\textwidth]{graphs/strong_scaling/strong_create_file.pdf}
\label{fig:l_ss_create_file}
}
\hspace{-8pt}
\subfigure[Create directory.] {
\includegraphics[width=0.19\textwidth]{graphs/strong_scaling/strong_mkdir.pdf}
\label{fig:l_ss_mkdir}
}

\label{fig:lambda_mds_strong_scaling}
\caption{Strong scaling comparison between {\proj} and HopsFS. The total total amount of vCPU allocated to {\proj} and HopsFS was varied between 16 and 512. For each vCPU value, both frameworks had the same number of clients, and each client performed 2,048 operations.}
\vspace{-15pt}
\end{center}
\end{figure*}
